Self-Adjusting Networks to Minimize Expected Path Length

Given a network infrastructure (e.g., data-center or on-chip-network) and a distribution on the source-destination requests, the expected path (route) length is an important measure for the performance, efficiency and power consumption of the network. In this work we initiate a study on self-adjusting networks: networks that use local-distributed mechanisms to adjust the position of the nodes (e.g., virtual machines) in the network to best fit the route requests distribution. Finding the optimal placement of nodes is defined as the minimum expected path length (MEPL) problem. This is a generalization of the minimum linear arrangement (MLA) problem where the network infrastructure is a line and the computation is done centrally. In contrast to previous work, we study the distributed version and give efficient and simple approximation algorithms for interesting and practically relevant special cases of the problem. In particular, we consider grid networks in which the distribution of requests is a symmetric product distribution. In this setting, we show that a simple greedy policy of position switching between neighboring nodes to locally minimize an objective function, achieves good approximation ratios. We are able to prove this result using the useful notions of expected rank of the distribution and the expected distance to the center of the graph.

==> ring_with_2_clusters.tex <==

\subsubsection{Scenario 1 -- worst case (need to be proved) local minimum}
\begin{itemize}
\item Ring with $n=c(2k+1)$ nodes, where $k$ -- some positive integer.
\item $c$ clusters -- $V_1, V_2, \ldots,V_c$ , where $\sum_{i=1}^c\left | V_i \right | =n$. 
\item Location of the nodes: $(v_1^1,v_1^2,v_1^3,\ldots,v_2^1,v_2^2,v_2^3,\ldots)$, where $v_i^j\in V_j$.
\item Uniform distribution of requests. I.e., activity level of each cluster is $p_i=1/c$ for $i\in{\{1,\ldots,c\}}$.
\end{itemize}



\begin{figure}
\begin{center}
\input{pics/ring1.tex}
\end{center}
\caption{Ring, with $2$ clusters each of size $2k+1$. In this case there are no improvement moves, i.e., the given placement is local minimum.}
\end{figure}


%\begin{figure}
%\begin{center}
%\input{pics/ring2.tex}
%\end{center}
%\caption{Ring, with $n=4k$.}
%\end{figure}
%
%
%\begin{figure}
%\label{fig_ring_optimal}
%\begin{center}
%\input{pics/ring3.tex}
%\end{center}
%\caption{Ring, with optimal nodes' placement.}
%\end{figure}



\begin{claim}\label{clm_scenario_1}
In scenario 1, the initial location of nodes $(v_1^1,v_1^2,v_1^3,\ldots,v_2^1,v_2^2,v_2^3,\ldots)$ is locally optimal, i.e., there are no improvement switches.
\end{claim}

\begin{proof}
First, let's denote the expected cost of the paths where the node $v$ is either source or destination as $\text{E}_v$. Due to the symmetric location and the uniform distribution, $\text{E}_v$ is the same for all the nodes $v\in V$. So, the expected path cost equals to $\text{E}_v$ for any $v\in V$. Let's assume that $v\in V_1$, where $V_1$ is the set of nodes in cluster $1$, and $\left| V_1\right |=2k+1$. Let's denote the probability of choosing the node $u\in{V_1}$ as a pair for the given node $v\in{V_1}$ as $p_{u|v}$. Clearly, $p_{u|v}=\frac{1}{|V_1|}$. 

\begin{align*}
\text{Before the switch: } \text{E}_v&=\sum_{u\in V_1}p_{u|v}d_{vu}\\
&= \frac{1}{\left| V_1\right |}\cdot 2\sum_{i=1}^k c\cdot i\\
&=\frac{c\cdot k(k+1)}{2k+1} 
\end{align*}

Due to the symmetry, there is no difference with what node we will try to switch the node $v$. So, let's assume that we switch it with its right-hand neighbor -- $w$. In order to check the difference with the path cost before the switch, we need to consider all the paths in which nodes $v$ and $w$ are involved. Clearly, even after the switch $\text{E}_v=\text{E}_w$ due to the symmetry, so we will now find the $\text{E}_v$ after the switch and will compare it to the $\text{E}_v$ before the switch.

\begin{align*}
\text{After the switch: } \text{E}_v&=\sum_{u\in V_1}p_{u|v}d_{vu}\\
&= \frac{1}{\left| V_1\right |}\left(\sum_{i=1}^k (c\cdot i-1)+\sum_{i=1}^k (c\cdot i+1)\right)\\
&=\frac{c\cdot k(k+1)}{2k+1} 
\end{align*}

Since all possible switches are the same due to the symmetry, we can conclude that there is no switch that will improve the expected paths cost.

\end{proof}



%\subsubsection{Scenario 2}
%Scenario 2 is identical to the scenario 1, but the total number of nodes now is: $n=4k$.
%
%\begin{claim}
%In scenario 2, the initial location of nodes $(v_1,u_1,v_2,u_2,v_3,u_3\ldots)$ is not locally optimal, i.e., there are improvement switches.
%\end{claim}
%
%\begin{proof}
%The proof is similar to the proof of Claim \ref{clm_scenario_1}. First, we calculate $\text{E}_v$ before the switch.
%
%\begin{align*}
%\text{Before the switch: } \text{E}_v=\sum_{u\in V_1}p_{vu}d_{vu}= \frac{1}{2\left| V_1\right |}(2\sum_{i=1}^{k-1} 2i + 2k)=\frac{2k^2}{2k}
%\end{align*}
%
%Now we switch the node $v$ with its right-hand neighbor $w$.
%
%\begin{align*}
%\text{After the switch: } \text{E}_v=\sum_{u\in V_1}p_{vu}d_{vu}= \frac{1}{2\left| V_1\right |}(1+2\sum_{i=2}^{k} 2i )=\frac{2k^2-1}{2k}
%\end{align*}
%
%Clearly, the switch between $u$ and $w$ yields smaller expected path. 
%
%\end{proof}


\subsubsection{Optimal locations for scenario 1}

Assume scenario 1 with the following location of the nodes:  $(v_1,v_2,...,v_{\left | V_1 \right |},u_1,u_2,...,u_{\left | V_2 \right |})$, where $v_i\in V_1$ and $u_i\in V_2$.

\begin{claim}
In scenario 1 with the following nodes' locations:  $(v_1^1,v_2^1,...,v_{\left | V_1 \right |}^1,v_1^2,v_2^2,...,v_{\left | V_2 \right |}^2,\ldots)$, where $v_i^j\in V_j$, the expected path cost is $\text{E}=\frac{k(2k+2)}{3(2k+1)}$.
\end{claim}

\begin{proof}
Let's consider the part of the ring of $2k+1$ nodes that belong to a single cluster. Number of paths of length 1 inside the cluster is $2\cdot 2k$. Number of paths of length 2 is $2\cdot (2k-1)$, length 3 is $2\cdot (2k-2)$, length $m$ is $2\cdot(2k-m+1)$, and of length $2k$ is $2$. So, we obtain the average path length in one cluster:

\begin{align*}
\text{E}&=\sum_{v,u\in V_1}p_{vu}d_{vu}\\
&= \frac{1}{2\left| V_1\right |^2}\cdot2\sum_{i=1}^{2k} m(2k-m+1)\\
&=\frac{k(2k+1)(4k+4)}{3\cdot 2(2k+1)^2}\\
&=\frac{k(2k+2)}{3(2k+1)}.
\end{align*}

\end{proof}


\begin{corollary}
The ratio between the worst case locations and the best case locations is $1.5c$, where $c$ is the number of clusters.
\end{corollary}

%\subsubsection{Open questions}
%
%\begin{itemize}
%
%\item Show that if $n=4k$ (so, there are improvement switches) then local switching strategy will converge to a global optimal solution.
%
%\item Show that scenario 1 is the worst case local minimum.
%
%\item Show that the local minimum is at most $x=?$ factor from the optimal solution.
%
%\item Show that the placement in Fig. \ref{fig_ring_optimal} is the optimal solution. Maybe just count paths: Total paths = total number of pairs. What is the maximum number of paths of length 1, length 2, ...
%
%\item Try to analyze the above scenarios, when the number of clusters is parameter. 
%
%\end{itemize}

